Quantum Transfer Learning for Real-World, Small, and High-Dimensional Datasets

Quantum machine learning (QML) networks promise to have some computational (or quantum) advantage for classifying supervised datasets (e.g., satellite images) over some conventional deep learning (DL) techniques due to their expressive power via their local effective dimension. There are, however, two main challenges regardless of the promised quantum advantage: 1) Currently available quantum bits (qubits) are very small in number, while real-world datasets are characterized by hundreds of high-dimensional elements (i.e., features). Additionally, there is not a single unified approach for embedding real-world high-dimensional datasets in a limited number of qubits. 2) Some real-world datasets are too small for training intricate QML networks. Hence, to tackle these two challenges for benchmarking and validating QML networks on real-world, small, and high-dimensional datasets in one-go, we employ quantum transfer learning composed of a multi-qubit QML network, and a very deep convolutional network (a with VGG16 architecture) extracting informative features from any small, high-dimensional dataset. We use real-amplitude and strongly-entangling N-layer QML networks with and without data re-uploading layers as a multi-qubit QML network, and evaluate their expressive power quantified by using their local effective dimension; the lower the local effective dimension of a QML network, the better its performance on unseen data. Our numerical results show that the strongly-entangling N-layer QML network has a lower local effective dimension than the real-amplitude QML network and outperforms it on the hard-to-classify three-class labelling problem. In addition, quantum transfer learning helps tackle the two challenges mentioned above for benchmarking and validating QML networks on real-world, small, and high-dimensional datasets.

==> colors.tex <==
\definecolor{sbblue}{rgb}{0.2823529411764706, 0.47058823529411764, 0.8156862745098039}
\definecolor{sborange}{rgb}{0.9333333333333333, 0.5215686274509804, 0.2901960784313726}
\definecolor{sbgreen}{rgb}{0.41568627450980394, 0.8, 0.39215686274509803}
\definecolor{sbred}{rgb}{0.8392156862745098, 0.37254901960784315, 0.37254901960784315}
\definecolor{sbpurple}{rgb}{0.5843137254901961, 0.4235294117647059, 0.7058823529411765}
\definecolor{sbbrown}{rgb}{0.5490196078431373, 0.3803921568627451, 0.23529411764705882}
\definecolor{sbmagenta}{rgb}{0.8627450980392157, 0.49411764705882355, 0.7529411764705882}
\definecolor{sbgray}{rgb}{0.4745098039215686, 0.4745098039215686, 0.4745098039215686}
\definecolor{sbocca}{rgb}{0.8352941176470589, 0.7333333333333333, 0.403921568627451}
\definecolor{sblightblue}{rgb}{0.5098039215686274, 0.7764705882352941, 0.8862745098039215}

\definecolor{lightgrey}{rgb}{0.9,0.9,0.9}
\definecolor{lightgreen}{RGB}{146,208,80}
\definecolor{lightblue}{RGB}{0,176,240}
\definecolor{darkgreen}{rgb}{0,0.39,0}

\definecolor{lightgreenblue}{RGB}{73,192,160}
\definecolor{VeryLightGray}{rgb}{0.9,0.9,0.9}
\definecolor{LightGray}{rgb}{0.8,0.8,0.8}
\definecolor{dlrgray}{RGB}{70,70,70}

\definecolor{dlightblue}{rgb}{0.65,0.65,0.98}
\definecolor{lightblue}{rgb}{0.85,0.85,1.0}
\definecolor{llightblue}{rgb}{0.95,0.95,0.98}
\definecolor{darkblue}{rgb}{0,0,.6}
\definecolor{darkred}{rgb}{.6,0,0}
\definecolor{lightred}{rgb}{1.0,0.75,0.75}
\definecolor{darkgreen}{rgb}{0,.6,0}
\definecolor{darkbrown}{rgb}{0.5,0.30,0.10}
\definecolor{grey}{rgb}{0.3,0.3,0.3}
\definecolor{red}{rgb}{.98,0,0}
\definecolor{hellgruen}{RGB}{146,208,80}
\definecolor{hellblau}{RGB}{0,176,240}
\definecolor{hellgruenblau}{RGB}{73,192,160}
\definecolor{VeryLightGray}{rgb}{0.9,0.9,0.9}
\definecolor{DLRgray}{RGB}{70,70,70}
\definecolor{dunkelblau}{RGB}{0,0,128}
\definecolor{dunkelgruen}{RGB}{0,128,0}
\definecolor{OvGUredMath}{RGB}{209,63,88}
\definecolor{AliceBlue}{rgb}{0.94,0.97,1}
\definecolor{BlueViolet}{rgb}{0.54,0.17,0.88}
\definecolor{CadetBlue}{rgb}{0.37,0.62,0.63}
\definecolor{CadetBlue1}{rgb}{0.59,0.96,1}
\definecolor{CadetBlue2}{rgb}{0.55,0.89,0.93}
\definecolor{CadetBlue3}{rgb}{0.48,0.77,0.8}
\definecolor{CadetBlue4}{rgb}{0.32,0.52,0.54}
\definecolor{CornflowerBlue}{rgb}{0.39,0.58,0.93}
\definecolor{DarkSlateBlue}{rgb}{0.28,0.24,0.54}
\definecolor{DarkTurquoise}{rgb}{0,0.8,0.82}
\definecolor{DeepSkyBlue}{rgb}{0,0.75,1}
\definecolor{DeepSkyBlue1}{rgb}{0,0.75,1}
\definecolor{DeepSkyBlue2}{rgb}{0,0.7,0.93}
\definecolor{DeepSkyBlue3}{rgb}{0,0.6,0.8}
\definecolor{DeepSkyBlue4}{rgb}{0,0.41,0.54}
\definecolor{DodgerBlue}{rgb}{0.12,0.56,1}
\definecolor{DodgerBlue1}{rgb}{0.12,0.56,1}
\definecolor{DodgerBlue2}{rgb}{0.11,0.52,0.93}
\definecolor{DodgerBlue3}{rgb}{0.09,0.45,0.8}
\definecolor{DodgerBlue4}{rgb}{0.06,0.3,0.54}
\definecolor{LightBlue}{rgb}{0.68,0.84,0.9}
\definecolor{LightBlue1}{rgb}{0.75,0.93,1}
\definecolor{LightBlue2}{rgb}{0.7,0.87,0.93}
\definecolor{LightBlue3}{rgb}{0.6,0.75,0.8}
\definecolor{LightBlue4}{rgb}{0.41,0.51,0.54}
\definecolor{LightCyan}{rgb}{0.88,1,1}
\definecolor{LightCyan1}{rgb}{0.88,1,1}
\definecolor{LightCyan2}{rgb}{0.82,0.93,0.93}
\definecolor{LightCyan3}{rgb}{0.7,0.8,0.8}
\definecolor{LightCyan4}{rgb}{0.48,0.54,0.54}
\definecolor{LightSkyBlue}{rgb}{0.53,0.8,0.98}
\definecolor{LightSkyBlue1}{rgb}{0.69,0.88,1}
\definecolor{LightSkyBlue2}{rgb}{0.64,0.82,0.93}
\definecolor{LightSkyBlue3}{rgb}{0.55,0.71,0.8}
\definecolor{LightSkyBlue4}{rgb}{0.38,0.48,0.54}
\definecolor{LightSlateBlue}{rgb}{0.52,0.44,1}
\definecolor{LightSteelBlue}{rgb}{0.69,0.77,0.87}
\definecolor{LightSteelBlue1}{rgb}{0.79,0.88,1}
\definecolor{LightSteelBlue2}{rgb}{0.73,0.82,0.93}
\definecolor{LightSteelBlue3}{rgb}{0.63,0.71,0.8}
\definecolor{LightSteelBlue4}{rgb}{0.43,0.48,0.54}
\definecolor{MediumAquamarine}{rgb}{0.4,0.8,0.66}
\definecolor{MediumBlue}{rgb}{0,0,0.8}
\definecolor{MediumSlateBlue}{rgb}{0.48,0.41,0.93}
\definecolor{MediumTurquoise}{rgb}{0.28,0.82,0.8}
\definecolor{MidnightBlue}{rgb}{0.1,0.1,0.44}
\definecolor{NavyBlue}{rgb}{0,0,0.5}
\definecolor{PaleTurquoise}{rgb}{0.68,0.93,0.93}
\definecolor{PaleTurquoise1}{rgb}{0.73,1,1}
\definecolor{PaleTurquoise2}{rgb}{0.68,0.93,0.93}
\definecolor{PaleTurquoise3}{rgb}{0.59,0.8,0.8}
\definecolor{PaleTurquoise4}{rgb}{0.4,0.54,0.54}
\definecolor{PowderBlue}{rgb}{0.69,0.88,0.9}
\definecolor{RoyalBlue}{rgb}{0.25,0.41,0.88}
\definecolor{RoyalBlue1}{rgb}{0.28,0.46,1}
\definecolor{RoyalBlue2}{rgb}{0.26,0.43,0.93}
\definecolor{RoyalBlue3}{rgb}{0.23,0.37,0.8}
\definecolor{RoyalBlue4}{rgb}{0.15,0.25,0.54}
\definecolor{SkyBlue}{rgb}{0.53,0.8,0.92}
\definecolor{SkyBlue1}{rgb}{0.53,0.8,1}
\definecolor{SkyBlue2}{rgb}{0.49,0.75,0.93}
\definecolor{SkyBlue3}{rgb}{0.42,0.65,0.8}
\definecolor{SkyBlue4}{rgb}{0.29,0.44,0.54}
\definecolor{SlateBlue}{rgb}{0.41,0.35,0.8}
\definecolor{SlateBlue1}{rgb}{0.51,0.43,1}
\definecolor{SlateBlue2}{rgb}{0.48,0.4,0.93}
\definecolor{SlateBlue3}{rgb}{0.41,0.35,0.8}
\definecolor{SlateBlue4}{rgb}{0.28,0.23,0.54}
\definecolor{SteelBlue}{rgb}{0.27,0.51,0.7}
\definecolor{SteelBlue1}{rgb}{0.39,0.72,1}
\definecolor{SteelBlue2}{rgb}{0.36,0.67,0.93}
\definecolor{SteelBlue3}{rgb}{0.31,0.58,0.8}
\definecolor{SteelBlue4}{rgb}{0.21,0.39,0.54}
\definecolor{aquamarine}{rgb}{0.5,1,0.83}
\definecolor{aquamarine1}{rgb}{0.5,1,0.83}
\definecolor{aquamarine2}{rgb}{0.46,0.93,0.77}
\definecolor{aquamarine3}{rgb}{0.4,0.8,0.66}
\definecolor{aquamarine4}{rgb}{0.27,0.54,0.45}
\definecolor{azure}{rgb}{0.94,1,1}
\definecolor{azure1}{rgb}{0.94,1,1}
\definecolor{azure2}{rgb}{0.88,0.93,0.93}
\definecolor{azure3}{rgb}{0.75,0.8,0.8}
\definecolor{azure4}{rgb}{0.51,0.54,0.54}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{blue1}{rgb}{0,0,1}
\definecolor{blue2}{rgb}{0,0,0.93}
\definecolor{blue3}{rgb}{0,0,0.8}
\definecolor{blue4}{rgb}{0,0,0.54}
\definecolor{cyan}{rgb}{0,1,1}
\definecolor{cyan1}{rgb}{0,1,1}
\definecolor{cyan2}{rgb}{0,0.93,0.93}
\definecolor{cyan3}{rgb}{0,0.8,0.8}
\definecolor{cyan4}{rgb}{0,0.54,0.54}
\definecolor{navy}{rgb}{0,0,0.5}
\definecolor{turquoise}{rgb}{0.25,0.88,0.81}
\definecolor{turquoise1}{rgb}{0,0.96,1}
\definecolor{turquoise2}{rgb}{0,0.89,0.93}
\definecolor{turquoise3}{rgb}{0,0.77,0.8}
\definecolor{turquoise4}{rgb}{0,0.52,0.54}
\definecolor{RosyBrown}{rgb}{0.73,0.56,0.56}
\definecolor{RosyBrown1}{rgb}{1,0.75,0.75}
\definecolor{RosyBrown2}{rgb}{0.93,0.7,0.7}
\definecolor{RosyBrown3}{rgb}{0.8,0.61,0.61}
\definecolor{RosyBrown4}{rgb}{0.54,0.41,0.41}
\definecolor{SaddleBrown}{rgb}{0.54,0.27,0.07}
\definecolor{SandyBrown}{rgb}{0.95,0.64,0.38}
\definecolor{beige}{rgb}{0.96,0.96,0.86}
\definecolor{brown}{rgb}{0.64,0.16,0.16}
\definecolor{brown1}{rgb}{1,0.25,0.25}
\definecolor{brown2}{rgb}{0.93,0.23,0.23}
\definecolor{brown3}{rgb}{0.8,0.2,0.2}
\definecolor{brown4}{rgb}{0.54,0.14,0.14}
\definecolor{burlywood}{rgb}{0.87,0.72,0.53}
\definecolor{burlywood1}{rgb}{1,0.82,0.61}
\definecolor{burlywood2}{rgb}{0.93,0.77,0.57}
\definecolor{burlywood3}{rgb}{0.8,0.66,0.49}
\definecolor{burlywood4}{rgb}{0.54,0.45,0.33}
\definecolor{chocolate}{rgb}{0.82,0.41,0.12}
\definecolor{chocolate1}{rgb}{1,0.5,0.14}
\definecolor{chocolate2}{rgb}{0.93,0.46,0.13}
\definecolor{chocolate3}{rgb}{0.8,0.4,0.11}
\definecolor{chocolate4}{rgb}{0.54,0.27,0.07}
\definecolor{peru}{rgb}{0.8,0.52,0.25}
\definecolor{tan}{rgb}{0.82,0.7,0.55}
\definecolor{tan1}{rgb}{1,0.64,0.31}
\definecolor{tan2}{rgb}{0.93,0.6,0.29}
\definecolor{tan3}{rgb}{0.8,0.52,0.25}
\definecolor{tan4}{rgb}{0.54,0.35,0.17}
\definecolor{DarkSlateGray}{rgb}{0.18,0.31,0.31}
\definecolor{DarkSlateGray1}{rgb}{0.59,1,1}
\definecolor{DarkSlateGray2}{rgb}{0.55,0.93,0.93}
\definecolor{DarkSlateGray3}{rgb}{0.47,0.8,0.8}
\definecolor{DarkSlateGray4}{rgb}{0.32,0.54,0.54}
\definecolor{DarkSlateGrey}{rgb}{0.18,0.31,0.31}
\definecolor{DimGray}{rgb}{0.41,0.41,0.41}
\definecolor{DimGrey}{rgb}{0.41,0.41,0.41}
\definecolor{LightGray}{rgb}{0.82,0.82,0.82}
\definecolor{LightGrey}{rgb}{0.82,0.82,0.82}
\definecolor{LightSlateGray}{rgb}{0.46,0.53,0.6}
\definecolor{LightSlateGrey}{rgb}{0.46,0.53,0.6}
\definecolor{SlateGray}{rgb}{0.44,0.5,0.56}
\definecolor{SlateGray1}{rgb}{0.77,0.88,1}
\definecolor{SlateGray2}{rgb}{0.72,0.82,0.93}
\definecolor{SlateGray3}{rgb}{0.62,0.71,0.8}
\definecolor{SlateGray4}{rgb}{0.42,0.48,0.54}
\definecolor{SlateGrey}{rgb}{0.44,0.5,0.56}
\definecolor{gray}{rgb}{0.74,0.74,0.74}
\definecolor{gray0}{rgb}{0,0,0}
\definecolor{gray1}{rgb}{0.01,0.01,0.01}
\definecolor{gray10}{rgb}{0.1,0.1,0.1}
\definecolor{DarkGreen}{rgb}{0,0.39,0}
\definecolor{DarkKhaki}{rgb}{0.74,0.71,0.42}
\definecolor{DarkOliveGreen}{rgb}{0.33,0.42,0.18}
\definecolor{DarkOliveGreen1}{rgb}{0.79,1,0.44}
\definecolor{DarkOliveGreen2}{rgb}{0.73,0.93,0.41}
\definecolor{DarkOliveGreen3}{rgb}{0.63,0.8,0.35}
\definecolor{DarkOliveGreen4}{rgb}{0.43,0.54,0.24}
\definecolor{DarkSeaGreen}{rgb}{0.56,0.73,0.56}
\definecolor{DarkSeaGreen1}{rgb}{0.75,1,0.75}
\definecolor{DarkSeaGreen2}{rgb}{0.7,0.93,0.7}
\definecolor{DarkSeaGreen3}{rgb}{0.61,0.8,0.61}
\definecolor{DarkSeaGreen4}{rgb}{0.41,0.54,0.41}
\definecolor{ForestGreen}{rgb}{0.13,0.54,0.13}
\definecolor{GreenYellow}{rgb}{0.68,1,0.18}
\definecolor{LawnGreen}{rgb}{0.48,0.98,0}
\definecolor{LightSeaGreen}{rgb}{0.13,0.7,0.66}
\definecolor{LimeGreen}{rgb}{0.2,0.8,0.2}
\definecolor{MediumSeaGreen}{rgb}{0.23,0.7,0.44}
\definecolor{MediumSpringGreen}{rgb}{0,0.98,0.6}
\definecolor{MintCream}{rgb}{0.96,1,0.98}
\definecolor{OliveDrab}{rgb}{0.42,0.55,0.14}
\definecolor{OliveDrab1}{rgb}{0.75,1,0.24}
\definecolor{OliveDrab2}{rgb}{0.7,0.93,0.23}
\definecolor{OliveDrab3}{rgb}{0.6,0.8,0.2}
\definecolor{OliveDrab4}{rgb}{0.41,0.54,0.13}
\definecolor{PaleGreen}{rgb}{0.59,0.98,0.59}
\definecolor{PaleGreen1}{rgb}{0.6,1,0.6}
\definecolor{PaleGreen2}{rgb}{0.56,0.93,0.56}
\definecolor{PaleGreen3}{rgb}{0.48,0.8,0.48}
\definecolor{PaleGreen4}{rgb}{0.33,0.54,0.33}
\definecolor{SeaGreen}{rgb}{0.18,0.54,0.34}
\definecolor{SeaGreen1}{rgb}{0.33,1,0.62}
\definecolor{SeaGreen2}{rgb}{0.3,0.93,0.58}
\definecolor{SeaGreen3}{rgb}{0.26,0.8,0.5}
\definecolor{SeaGreen4}{rgb}{0.18,0.54,0.34}
\definecolor{SpringGreen}{rgb}{0,1,0.5}
\definecolor{SpringGreen1}{rgb}{0,1,0.5}
\definecolor{SpringGreen2}{rgb}{0,0.93,0.46}
\definecolor{SpringGreen3}{rgb}{0,0.8,0.4}
\definecolor{SpringGreen4}{rgb}{0,0.54,0.27}
\definecolor{YellowGreen}{rgb}{0.6,0.8,0.2}
\definecolor{chartreuse}{rgb}{0.5,1,0}
\definecolor{chartreuse1}{rgb}{0.5,1,0}
\definecolor{chartreuse2}{rgb}{0.46,0.93,0}
\definecolor{chartreuse3}{rgb}{0.4,0.8,0}
\definecolor{chartreuse4}{rgb}{0.27,0.54,0}
\definecolor{green}{rgb}{0,1,0}
\definecolor{green1}{rgb}{0,1,0}
\definecolor{green2}{rgb}{0,0.93,0}
\definecolor{green3}{rgb}{0,0.8,0}
\definecolor{green4}{rgb}{0,0.54,0}
\definecolor{khaki}{rgb}{0.94,0.9,0.55}
\definecolor{khaki1}{rgb}{1,0.96,0.56}
\definecolor{khaki2}{rgb}{0.93,0.9,0.52}
\definecolor{khaki3}{rgb}{0.8,0.77,0.45}
\definecolor{khaki4}{rgb}{0.54,0.52,0.3}
\definecolor{DarkOrange}{rgb}{1,0.55,0}
\definecolor{DarkOrange1}{rgb}{1,0.5,0}
\definecolor{DarkOrange2}{rgb}{0.93,0.46,0}
\definecolor{DarkOrange3}{rgb}{0.8,0.4,0}
\definecolor{DarkOrange4}{rgb}{0.54,0.27,0}
\definecolor{DarkSalmon}{rgb}{0.91,0.59,0.48}
\definecolor{LightCoral}{rgb}{0.94,0.5,0.5}
\definecolor{LightSalmon}{rgb}{1,0.63,0.48}
\definecolor{LightSalmon1}{rgb}{1,0.63,0.48}
\definecolor{LightSalmon2}{rgb}{0.93,0.58,0.45}
\definecolor{LightSalmon3}{rgb}{0.8,0.5,0.38}
\definecolor{LightSalmon4}{rgb}{0.54,0.34,0.26}
\definecolor{PeachPuff}{rgb}{1,0.85,0.72}
\definecolor{PeachPuff1}{rgb}{1,0.85,0.72}
\definecolor{PeachPuff2}{rgb}{0.93,0.79,0.68}
\definecolor{PeachPuff3}{rgb}{0.8,0.68,0.58}
\definecolor{PeachPuff4}{rgb}{0.54,0.46,0.39}
\definecolor{bisque}{rgb}{1,0.89,0.77}
\definecolor{bisque1}{rgb}{1,0.89,0.77}
\definecolor{bisque2}{rgb}{0.93,0.83,0.71}
\definecolor{bisque3}{rgb}{0.8,0.71,0.62}
\definecolor{bisque4}{rgb}{0.54,0.49,0.42}
\definecolor{coral}{rgb}{1,0.5,0.31}
\definecolor{coral1}{rgb}{1,0.45,0.34}
\definecolor{coral2}{rgb}{0.93,0.41,0.31}
\definecolor{coral3}{rgb}{0.8,0.36,0.27}
\definecolor{coral4}{rgb}{0.54,0.24,0.18}
\definecolor{honeydew}{rgb}{0.94,1,0.94}
\definecolor{honeydew1}{rgb}{0.94,1,0.94}
\definecolor{honeydew2}{rgb}{0.88,0.93,0.88}
\definecolor{honeydew3}{rgb}{0.75,0.8,0.75}
\definecolor{honeydew4}{rgb}{0.51,0.54,0.51}
\definecolor{orange}{rgb}{1,0.64,0}
\definecolor{orange1}{rgb}{1,0.64,0}
\definecolor{orange2}{rgb}{0.93,0.6,0}
\definecolor{orange3}{rgb}{0.8,0.52,0}
\definecolor{orange4}{rgb}{0.54,0.35,0}
\definecolor{salmon}{rgb}{0.98,0.5,0.45}
\definecolor{salmon1}{rgb}{1,0.55,0.41}
\definecolor{salmon2}{rgb}{0.93,0.51,0.38}
\definecolor{salmon3}{rgb}{0.8,0.44,0.33}
\definecolor{salmon4}{rgb}{0.54,0.3,0.22}
\definecolor{sienna}{rgb}{0.63,0.32,0.18}
\definecolor{sienna1}{rgb}{1,0.51,0.28}
\definecolor{sienna2}{rgb}{0.93,0.47,0.26}
\definecolor{sienna3}{rgb}{0.8,0.41,0.22}
\definecolor{sienna4}{rgb}{0.54,0.28,0.15}
\definecolor{DeepPink}{rgb}{1,0.08,0.57}
\definecolor{DeepPink1}{rgb}{1,0.08,0.57}
\definecolor{DeepPink2}{rgb}{0.93,0.07,0.54}
\definecolor{DeepPink3}{rgb}{0.8,0.06,0.46}
\definecolor{DeepPink4}{rgb}{0.54,0.04,0.31}
\definecolor{HotPink}{rgb}{1,0.41,0.7}
\definecolor{HotPink1}{rgb}{1,0.43,0.7}
\definecolor{HotPink2}{rgb}{0.93,0.41,0.65}
\definecolor{HotPink3}{rgb}{0.8,0.38,0.56}
\definecolor{HotPink4}{rgb}{0.54,0.23,0.38}
\definecolor{IndianRed}{rgb}{0.8,0.36,0.36}
\definecolor{IndianRed1}{rgb}{1,0.41,0.41}
\definecolor{IndianRed2}{rgb}{0.93,0.39,0.39}
\definecolor{IndianRed3}{rgb}{0.8,0.33,0.33}
\definecolor{IndianRed4}{rgb}{0.54,0.23,0.23}
\definecolor{LightPink}{rgb}{1,0.71,0.75}
\definecolor{LightPink1}{rgb}{1,0.68,0.72}
\definecolor{LightPink2}{rgb}{0.93,0.63,0.68}
\definecolor{LightPink3}{rgb}{0.8,0.55,0.58}
\definecolor{LightPink4}{rgb}{0.54,0.37,0.39}
\definecolor{MediumVioletRed}{rgb}{0.78,0.08,0.52}
\definecolor{MistyRose}{rgb}{1,0.89,0.88}
\definecolor{MistyRose1}{rgb}{1,0.89,0.88}
\definecolor{MistyRose2}{rgb}{0.93,0.83,0.82}
\definecolor{MistyRose3}{rgb}{0.8,0.71,0.71}
\definecolor{MistyRose4}{rgb}{0.54,0.49,0.48}
\definecolor{OrangeRed}{rgb}{1,0.27,0}
\definecolor{OrangeRed1}{rgb}{1,0.27,0}
\definecolor{OrangeRed2}{rgb}{0.93,0.25,0}
\definecolor{OrangeRed3}{rgb}{0.8,0.21,0}
\definecolor{OrangeRed4}{rgb}{0.54,0.14,0}
\definecolor{PaleVioletRed}{rgb}{0.86,0.44,0.57}
\definecolor{PaleVioletRed1}{rgb}{1,0.51,0.67}
\definecolor{PaleVioletRed2}{rgb}{0.93,0.47,0.62}
\definecolor{PaleVioletRed3}{rgb}{0.8,0.41,0.54}
\definecolor{PaleVioletRed4}{rgb}{0.54,0.28,0.36}
\definecolor{VioletRed}{rgb}{0.81,0.13,0.56}
\definecolor{VioletRed1}{rgb}{1,0.24,0.59}
\definecolor{VioletRed2}{rgb}{0.93,0.23,0.55}
\definecolor{VioletRed3}{rgb}{0.8,0.2,0.47}
\definecolor{VioletRed4}{rgb}{0.54,0.13,0.32}
\definecolor{firebrick}{rgb}{0.7,0.13,0.13}
\definecolor{firebrick1}{rgb}{1,0.19,0.19}
\definecolor{firebrick2}{rgb}{0.93,0.17,0.17}
\definecolor{firebrick3}{rgb}{0.8,0.15,0.15}
\definecolor{firebrick4}{rgb}{0.54,0.1,0.1}
\definecolor{pink}{rgb}{1,0.75,0.79}
\definecolor{pink1}{rgb}{1,0.71,0.77}
\definecolor{pink2}{rgb}{0.93,0.66,0.72}
\definecolor{pink3}{rgb}{0.8,0.57,0.62}
\definecolor{pink4}{rgb}{0.54,0.39,0.42}
\definecolor{red}{rgb}{1,0,0}
\definecolor{red1}{rgb}{1,0,0}
\definecolor{red2}{rgb}{0.93,0,0}
\definecolor{red3}{rgb}{0.8,0,0}
\definecolor{red4}{rgb}{0.54,0,0}
\definecolor{tomato}{rgb}{1,0.39,0.28}
\definecolor{tomato1}{rgb}{1,0.39,0.28}
\definecolor{tomato2}{rgb}{0.93,0.36,0.26}
\definecolor{tomato3}{rgb}{0.8,0.31,0.22}
\definecolor{tomato4}{rgb}{0.54,0.21,0.15}
\definecolor{DarkOrchid}{rgb}{0.6,0.2,0.8}
\definecolor{DarkOrchid1}{rgb}{0.75,0.24,1}
\definecolor{DarkOrchid2}{rgb}{0.7,0.23,0.93}
\definecolor{DarkOrchid3}{rgb}{0.6,0.2,0.8}
\definecolor{DarkOrchid4}{rgb}{0.41,0.13,0.54}
\definecolor{DarkViolet}{rgb}{0.58,0,0.82}
\definecolor{LavenderBlush}{rgb}{1,0.94,0.96}
\definecolor{LavenderBlush1}{rgb}{1,0.94,0.96}
\definecolor{LavenderBlush2}{rgb}{0.93,0.88,0.89}
\definecolor{LavenderBlush3}{rgb}{0.8,0.75,0.77}
\definecolor{LavenderBlush4}{rgb}{0.54,0.51,0.52}
\definecolor{MediumOrchid}{rgb}{0.73,0.33,0.82}
\definecolor{MediumOrchid1}{rgb}{0.88,0.4,1}
\definecolor{MediumOrchid2}{rgb}{0.82,0.37,0.93}
\definecolor{MediumOrchid3}{rgb}{0.7,0.32,0.8}
\definecolor{MediumOrchid4}{rgb}{0.48,0.21,0.54}
\definecolor{MediumPurple}{rgb}{0.57,0.44,0.86}
\definecolor{MediumPurple1}{rgb}{0.67,0.51,1}
\definecolor{MediumPurple2}{rgb}{0.62,0.47,0.93}
\definecolor{MediumPurple3}{rgb}{0.54,0.41,0.8}
\definecolor{MediumPurple4}{rgb}{0.36,0.28,0.54}
\definecolor{lavender}{rgb}{0.9,0.9,0.98}
\definecolor{magenta}{rgb}{1,0,1}
\definecolor{magenta1}{rgb}{1,0,1}
\definecolor{magenta2}{rgb}{0.93,0,0.93}
\definecolor{magenta3}{rgb}{0.8,0,0.8}
\definecolor{magenta4}{rgb}{0.54,0,0.54}
\definecolor{maroon}{rgb}{0.69,0.19,0.38}
\definecolor{maroon1}{rgb}{1,0.2,0.7}
\definecolor{maroon2}{rgb}{0.93,0.19,0.65}
\definecolor{maroon3}{rgb}{0.8,0.16,0.56}
\definecolor{maroon4}{rgb}{0.54,0.11,0.38}
\definecolor{orchid}{rgb}{0.85,0.44,0.84}
\definecolor{orchid1}{rgb}{1,0.51,0.98}
\definecolor{orchid2}{rgb}{0.93,0.48,0.91}
\definecolor{orchid3}{rgb}{0.8,0.41,0.79}
\definecolor{orchid4}{rgb}{0.54,0.28,0.54}
\definecolor{plum}{rgb}{0.86,0.63,0.86}
\definecolor{plum1}{rgb}{1,0.73,1}
\definecolor{plum2}{rgb}{0.93,0.68,0.93}
\definecolor{plum3}{rgb}{0.8,0.59,0.8}
\definecolor{plum4}{rgb}{0.54,0.4,0.54}
\definecolor{purple}{rgb}{0.63,0.13,0.94}
\definecolor{purple1}{rgb}{0.61,0.19,1}
\definecolor{purple2}{rgb}{0.57,0.17,0.93}
\definecolor{purple3}{rgb}{0.49,0.15,0.8}
\definecolor{purple4}{rgb}{0.33,0.1,0.54}
\definecolor{thistle}{rgb}{0.84,0.75,0.84}
\definecolor{thistle1}{rgb}{1,0.88,1}
\definecolor{thistle2}{rgb}{0.93,0.82,0.93}
\definecolor{thistle3}{rgb}{0.8,0.71,0.8}
\definecolor{thistle4}{rgb}{0.54,0.48,0.54}
\definecolor{violet}{rgb}{0.93,0.51,0.93}
\definecolor{AntiqueWhite}{rgb}{0.98,0.92,0.84}
\definecolor{AntiqueWhite1}{rgb}{1,0.93,0.86}
\definecolor{AntiqueWhite2}{rgb}{0.93,0.87,0.8}
\definecolor{AntiqueWhite3}{rgb}{0.8,0.75,0.69}
\definecolor{AntiqueWhite4}{rgb}{0.54,0.51,0.47}
\definecolor{FloralWhite}{rgb}{1,0.98,0.94}
\definecolor{GhostWhite}{rgb}{0.97,0.97,1}
\definecolor{NavajoWhite}{rgb}{1,0.87,0.68}
\definecolor{NavajoWhite1}{rgb}{1,0.87,0.68}
\definecolor{NavajoWhite2}{rgb}{0.93,0.81,0.63}
\definecolor{NavajoWhite3}{rgb}{0.8,0.7,0.54}
\definecolor{NavajoWhite4}{rgb}{0.54,0.47,0.37}
\definecolor{OldLace}{rgb}{0.99,0.96,0.9}
\definecolor{WhiteSmoke}{rgb}{0.96,0.96,0.96}
\definecolor{gainsboro}{rgb}{0.86,0.86,0.86}
\definecolor{ivory}{rgb}{1,1,0.94}
\definecolor{ivory1}{rgb}{1,1,0.94}
\definecolor{ivory2}{rgb}{0.93,0.93,0.88}
\definecolor{ivory3}{rgb}{0.8,0.8,0.75}
\definecolor{ivory4}{rgb}{0.54,0.54,0.51}
\definecolor{linen}{rgb}{0.98,0.94,0.9}
\definecolor{seashell}{rgb}{1,0.96,0.93}
\definecolor{seashell1}{rgb}{1,0.96,0.93}
\definecolor{seashell2}{rgb}{0.93,0.89,0.87}
\definecolor{seashell3}{rgb}{0.8,0.77,0.75}
\definecolor{seashell4}{rgb}{0.54,0.52,0.51}
\definecolor{snow}{rgb}{1,0.98,0.98}
\definecolor{snow1}{rgb}{1,0.98,0.98}
\definecolor{snow2}{rgb}{0.93,0.91,0.91}
\definecolor{snow3}{rgb}{0.8,0.79,0.79}
\definecolor{snow4}{rgb}{0.54,0.54,0.54}
\definecolor{wheat}{rgb}{0.96,0.87,0.7}
\definecolor{wheat1}{rgb}{1,0.9,0.73}
\definecolor{wheat2}{rgb}{0.93,0.84,0.68}
\definecolor{wheat3}{rgb}{0.8,0.73,0.59}
\definecolor{wheat4}{rgb}{0.54,0.49,0.4}
\definecolor{white}{rgb}{1,1,1}
\definecolor{BlanchedAlmond}{rgb}{1,0.92,0.8}
\definecolor{DarkGoldenrod}{rgb}{0.72,0.52,0.04}
\definecolor{DarkGoldenrod1}{rgb}{1,0.72,0.06}
\definecolor{DarkGoldenrod2}{rgb}{0.93,0.68,0.05}
\definecolor{DarkGoldenrod3}{rgb}{0.8,0.58,0.05}
\definecolor{DarkGoldenrod4}{rgb}{0.54,0.39,0.03}
\definecolor{LemonChiffon}{rgb}{1,0.98,0.8}
\definecolor{LemonChiffon1}{rgb}{1,0.98,0.8}
\definecolor{LemonChiffon2}{rgb}{0.93,0.91,0.75}
\definecolor{LemonChiffon3}{rgb}{0.8,0.79,0.64}
\definecolor{LemonChiffon4}{rgb}{0.54,0.54,0.44}
\definecolor{LightGoldenrod}{rgb}{0.93,0.86,0.51}
\definecolor{LightGoldenrod1}{rgb}{1,0.92,0.54}
\definecolor{LightGoldenrod2}{rgb}{0.93,0.86,0.51}
\definecolor{LightGoldenrod3}{rgb}{0.8,0.74,0.44}
\definecolor{LightGoldenrod4}{rgb}{0.54,0.5,0.3}
\definecolor{LightGoldenrodYellow}{rgb}{0.98,0.98,0.82}
\definecolor{LightYellow}{rgb}{1,1,0.88}
\definecolor{LightYellow1}{rgb}{1,1,0.88}
\definecolor{LightYellow2}{rgb}{0.93,0.93,0.82}
\definecolor{LightYellow3}{rgb}{0.8,0.8,0.7}
\definecolor{LightYellow4}{rgb}{0.54,0.54,0.48}
\definecolor{PaleGoldenrod}{rgb}{0.93,0.91,0.66}
\definecolor{PapayaWhip}{rgb}{1,0.93,0.83}
\definecolor{cornsilk}{rgb}{1,0.97,0.86}
\definecolor{cornsilk1}{rgb}{1,0.97,0.86}
\definecolor{cornsilk2}{rgb}{0.93,0.91,0.8}
\definecolor{cornsilk3}{rgb}{0.8,0.78,0.69}
\definecolor{cornsilk4}{rgb}{0.54,0.53,0.47}
\definecolor{gold}{rgb}{1,0.84,0}
\definecolor{gold1}{rgb}{1,0.84,0}
\definecolor{gold2}{rgb}{0.93,0.79,0}
\definecolor{gold3}{rgb}{0.8,0.68,0}
\definecolor{gold4}{rgb}{0.54,0.46,0}
\definecolor{goldenrod}{rgb}{0.85,0.64,0.13}
\definecolor{goldenrod1}{rgb}{1,0.75,0.14}
\definecolor{goldenrod2}{rgb}{0.93,0.7,0.13}
\definecolor{goldenrod3}{rgb}{0.8,0.61,0.11}
\definecolor{goldenrod4}{rgb}{0.54,0.41,0.08}
\definecolor{moccasin}{rgb}{1,0.89,0.71}
\definecolor{yellow}{rgb}{1,1,0}
\definecolor{yellow1}{rgb}{1,1,0}
\definecolor{yellow2}{rgb}{0.93,0.93,0}
\definecolor{yellow3}{rgb}{0.8,0.8,0}
\definecolor{yellow4}{rgb}{0.54,0.54,0}

